Assembly of FETI dual operator using CUDA

FETI is a numerical method used to solve engineering problems. It builds on the ideas of domain decomposition, which makes it highly scalable and capable of efficiently utilizing whole supercomputers. One of the most time-consuming parts of the FETI solver is the application of the dual operator F in every iteration of the solver. It is traditionally performed on the CPU using an implicit approach of applying the individual sparse matrices that form F right-to-left. Another approach is to apply the dual operator explicitly, which primarily involves a simple dense matrix-vector multiplication and can be efficiently performed on the GPU. However, this requires additional preprocessing on the CPU where the dense matrix is assembled, which makes the explicit approach beneficial only after hundreds of iterations are performed. In this paper, we use the GPU to accelerate the assembly process as well. This significantly shortens the preprocessing time, thus decreasing the number of solver iterations needed to make the explicit approach beneficial. With a proper configuration, we only need a few tens of iterations to achieve speedup relative to the implicit CPU approach. Compared to the CPU-only explicit approach, we achieved up to 10x speedup for the preprocessing and 25x for the application.

==> tikz/settings/solve_type.tex <==
\begin{tikzpicture}
  \begin{loglogaxis}[
    log basis x=2,
    log basis y=10,
    xlabel={Number of DOFs per subdomain},
    ylabel={Time per subdomain [ms]},
    xmajorgrids=true,
    ymajorgrids=true,
    every axis plot/.append style={line width=1.2pt},
    grid style=dotted,
    xmin=45,
    xmax=97469,
    ymin=87.328,
    ymax=19411,
    label style={font=\footnotesize},
    tick label style={font=\footnotesize},
    legend style={font=\footnotesize, draw=none, at={(0.5,-0.18)}, anchor=north, legend columns=-1},
    legend cell align={left}
  ]
    \addplot[solid, color={red}, mark=none] coordinates {
      (    64 ,   128.484 )
      (   125 ,   251.049 )
      (   216 ,   518.588 )
      (   343 ,   835.413 )
      (   729 ,  2739.623 )
      (  1331 ,  3792.951 )
      (  2744 ,  5857.602 )
      (  4913 ,  6683.674 )
      (  9261 ,  8259.659 )
      ( 17576 , 13675.048 )
    };
    \addplot[dashed, color={blue}, mark=none] coordinates {
      (    64 ,   123.832 )
      (   125 ,   255.126 )
      (   216 ,   518.297 )
      (   343 ,   837.585 )
      (   729 ,  2733.627 )
      (  1331 ,  3803.600 )
      (  2744 ,  5894.557 )
      (  4913 ,  6694.798 )
      (  9261 ,  8283.735 )
      ( 17576 , 13726.117 )
    };
    \addlegendentry{L}
    \addlegendentry{LHH}
  \end{loglogaxis}
\end{tikzpicture}

